Sampling Bag of Views for Open-Vocabulary Object Detection

Existing open-vocabulary object detection (OVD) develops methods for testing unseen categories by aligning object region embeddings with corresponding VLM features. A recent study leverages the idea that VLMs implicitly learn compositional structures of semantic concepts within the image. Instead of using an individual region embedding, it utilizes a bag of region embeddings as a new representation to incorporate compositional structures into the OVD task. However, this approach often fails to capture the contextual concepts of each region, leading to noisy compositional structures. This results in only marginal performance improvements and reduced efficiency. To address this, we propose a novel concept-based alignment method that samples a more powerful and efficient compositional structure. Our approach groups contextually related ``concepts'' into a bag and adjusts the scale of concepts within the bag for more effective embedding alignment. Combined with Faster R-CNN, our method achieves improvements of 2.6 box AP50 and 0.5 mask AP over prior work on novel categories in the open-vocabulary COCO and LVIS benchmarks. Furthermore, our method reduces CLIP computation in FLOPs by 80.3% compared to previous research, significantly enhancing efficiency. Experimental results demonstrate that the proposed method outperforms previous state-of-the-art models on the OVD datasets.

==> sec/Y_trash_bin.tex <==
% \noindent \textbf{Exploring Vision-Language Alignment.}

% Vision-language pre-training aims to learn alignment between image and text representations by leveraging vision-language models (VLMs) \cite{CLIP} trained on large-scale image-text pairs for segmentation and detection \cite{OVOD, OVR-CNN, BARON}. There are many studies \cite{ViLT, BLIP, ABF, Vilbert} that pre-train VLMs to improve the performance of downstream recognition and generation tasks. There are also studies \cite{DVDet, SHiNe, ContextDET} that enhance image-text alignment by enriching text prompts with guidance from Large Language Models (LLMs). Some studies push forward in another direction by strengthening image representations. CoDet \cite{CoDet} identifies key region proposals for query text by using visual clues (\eg object co-occurrence) in image-text pairs with the same concept. CLIM \cite{CLIM} employs mosaic augmentation by combining multiple batch images into one. The mosaicked images are trained with contrastive loss to match the corresponding text embeddings while dissimilar from others. InstaGen \cite{InstaGen} enhances the ability of object detectors by utilizing synthesized images from generative models for novel class prediction. However, these CLIP-based OVD methods require external knowledge, such as additional data or tools (\eg generative models or LLMs).

% BARON \cite{BARON} detours these constraints by sampling the nearest neighbors around each region proposal within an image. It enables VLMs to infer the compositional structure of semantic concepts without relying on external knowledge. MaskCLIP \cite{MaskCLIP} demonstrates this, showing that VLMs \cite{BERT, CLIP, SAM} effectively capture representations of concepts in complex scenes that are not explicitly learned. Specifically, VLMs implicitly learn the compositional structure of complex scenes from large-scale image-text pairs, aligning each concept's pixel embedding with its corresponding text representation. Nevertheless, BARON's reliance on probabilistic sampling of surrounding neighbors leads to high computational costs and sub-optimal performance. This motivates us to explore an efficient and powerful compositional structure of semantic concepts. We aim to achieve this by allowing the compositional structure to capture nearby co-occurring concepts accurately. This applies without relying on external knowledge (\eg extra foundation models).

% To extract key concepts from these candidates, we build a canvas $\mathcal{C}$--—a graph structure where vertices represent region proposals, edges $\boldsymbol{\mathcal{E}}$ represent semantically related visual concepts, and coordinates encode the likelihood of nearby RPN boxes. At each coordinate, these probabilities are calculated by summing the objectness score of nearby candidates based on their spatial proximity. $\boldsymbol{\mathcal{E}}$ are extracted through probabilistic exploration between all region proposals in $\mathcal{C}$. This enables converging on a few informative concepts near region proposals. In \cref{fig:1_teaser}-b, we then form a \textit{bag of concepts} by adjusting neighboring boxes to incorporate $\boldsymbol{\mathcal{E}}$ in their direction. This adaptive sampling strategy better recognizes the compositional structure and improves the efficiency of VLMs.


% If the local view is small, selecting a broader view (such as the global or middle view) can increase scene complexity. Conversely, if the parent contains more co-occurring concepts, it better captures compositional structure.
